Measure-Theoretic Anti-Causal Representation Learning

Causal representation learning in the anti-causal setting (labels cause features rather than the reverse) presents unique challenges requiring specialized approaches. We propose Anti-Causal Invariant Abstractions (ACIA), a novel measure-theoretic framework for anti-causal representation learning. ACIA employs a two-level design, low-level representations capture how labels generate observations, while high-level representations learn stable causal patterns across environment-specific variations. ACIA addresses key limitations of existing approaches by accommodating prefect and imperfect interventions through interventional kernels, eliminating dependency on explicit causal structures, handling high-dimensional data effectively, and providing theoretical guarantees for out-of-distribution generalization. Experiments on synthetic and real-world medical datasets demonstrate that ACIA consistently outperforms state-of-the-art methods in both accuracy and invariance metrics. Furthermore, our theoretical results establish tight bounds on performance gaps between training and unseen environments, confirming the efficacy of our approach for robust anti-causal learning.

==> macros.tex <==
\allowdisplaybreaks
% \usepackage{cite}
\usepackage{graphicx}
\usepackage{tikz}
\usepackage{tikz-cd}
\usepackage{times}
\usepackage{courier}
\usepackage{bm}
\usepackage{physics}
\usepackage{xcolor}
\usepackage{natbib}
\usepackage{mdframed}
\usepackage{nicefrac}
\usepackage{booktabs}
\usepackage{lipsum}
\usepackage{titlesec}
\usepackage{wrapfig,lipsum,booktabs}
\usepackage{authblk}
\usepackage{blindtext}


\usepackage{algorithm}
\usepackage{algpseudocode}
% Algorithm definitions
\newcommand{\commentsymbol}{//}% or \% or $\triangleright$
\algrenewcommand\algorithmiccomment[1]{\hfill {\footnotesize \commentsymbol{} #1}}




\usepackage{titletoc}
\usepackage{todonotes}
\usepackage{authblk}
\usepackage{setspace}
\usepackage{dsfont} % for \mathbb{1} as \mathds{1}
\newcommand{\one}{\mathds{1}}

%%% Section Notation %%%
\usepackage[nameinlink,capitalize,noabbrev]{cleveref}
% \crefformat{section}{\S#2#1#3} % see manual of cleveref, section 8.2.1
% \crefformat{subsection}{\S#2#1#3}
% \crefformat{subsubsection}{\S#2#1#3}
% \crefformat{appendix}{\S #2#1#3}
% use: See \cref{sec:section}, \cref{sec:subsection} or \cref{sec:subsubsection}
%%% Section Notation %%%

%%% Chinese ###
\usepackage{CJK}
\newcommand{\zh}[1]{\begin{CJK}{UTF8}{bsmi}\normalfont\small #1\end{CJK}} % 繁體中文
\newcommand{\zhs}[1]{\begin{CJK}{UTF8}{gbsn}\normalfont \small#1\end{CJK}}% 簡體中文 
%%%% \begin{CJK}{UTF8}{bsmi}\normalfont 中文\end{CJK} when word missing %%%

%%%Claim%%%
\newenvironment{claim}{  \begin{mdframed}[linecolor=black!0,backgroundcolor=black!10]\noindent%\itshape
		\ignorespaces}{\end{mdframed}}

% \let\originalfigure=\figure
% \let\endoriginalfigure=\endfigure

% \renewenvironment{figure}[1][]{
%   \begin{originalfigure}[#1]
%     \begin{mdframed}[linecolor=black!0,backgroundcolor=black!1]
% }{
%     \end{mdframed}
%   \end{originalfigure}
% }
%%%Claim%%%

%%%% skip line in table %%%
\usepackage{array}
\usepackage{makecell}

\renewcommand\theadalign{bc}
\renewcommand\theadfont{\bfseries}
\renewcommand\theadgape{\Gape[4pt]}
\renewcommand\cellgape{\Gape[0pt]}
%%%% skip line in table %%%

%% Comment%%
\newcommand{\jerry}[1]{\textcolor{firebrick}{[JH: #1]}}
%%Comment%%
%%%theorem%%%
% \newenvironment{theorem}{  \begin{mdframed}[linecolor=black]\noindent\ignorespaces}{\end{mdframed}}
%%%theorem%%%

\def\half{{\frac{1}{2}}}

\def\({\left(}
\def\){\right)}
\def\[{\left[}
\def\]{\right]}


%

\usepackage{dashbox}
\usepackage{xcolor}
\usepackage{colortbl}
\definecolor{lightyellow}{rgb}{1.0, 0.95, 0.7}
% \definecolor{Blue}{rgb}{0, 0.18, 0.65}
\definecolor{Blue}{rgb}{0, 0, 0.8}
\definecolor{blue}{rgb}{0,0,1}
% \definecolor{darkgreen}{rgb}{0.01,0.50,0.2}
\definecolor{darkgreen}{rgb}{0,0.40,0}
\definecolor{firebrick}{rgb}{0.698,0.133,0.133}
\newcommand*{\red}[1]{\textcolor{red}{#1}}
\newcommand*{\Red}[1]{\textcolor{firebrick}{#1}}
\newcommand*{\Blue}[1]{\textcolor{Blue}{#1}}
\newcommand*{\blue}[1]{\textcolor{blue}{#1}}
\newcommand*{\green}[1]{\textcolor{darkgreen}{#1}}
\newcommand*{\black}[1]{\textcolor{black}{#1}}

\definecolor{colorA}{rgb}{1,0,0}
\definecolor{colorB}{rgb}{0,0.3,1}
\definecolor{colorC}{rgb}{0.9,0.8,0.2}
\definecolor{colorD}{rgb}{0,0.65,0}
\definecolor{lesslightgray}{rgb}{0.5,0.5,0.5}
\definecolor{light-gray}{gray}{0.95}
\newcommand{\code}[1]{\colorbox{light-gray}{\footnotesize\texttt{#1}}}
\newcommand*{\grey}[1]{\textcolor{black!50}{#1}}
\newcommand*{\colorA}[1]{\textcolor{colorA}{#1}}
\newcommand*{\colorB}[1]{\textcolor{colorB}{#1}}
\newcommand*{\colorC}[1]{\textcolor{colorC}{#1}}
\newcommand*{\colorD}[1]{\textcolor{colorD}{#1}}


\let\tilde\widetilde
\let\hat\widehat

\newcommand{\calA}{\mathcal{A}}
\newcommand{\calB}{\mathcal{B}}
\newcommand{\calC}{\mathcal{C}}
\newcommand{\calD}{\mathcal{D}}
\newcommand{\calE}{\mathcal{E}}
\newcommand{\calF}{\mathcal{F}}
\newcommand{\calG}{\mathcal{G}}
\newcommand{\calH}{\mathcal{H}}
\newcommand{\calI}{\mathcal{I}}
\newcommand{\calJ}{\mathcal{J}}
\newcommand{\calK}{\mathcal{K}}
\newcommand{\calL}{\mathcal{L}}
\newcommand{\calM}{\mathcal{M}}
\newcommand{\calN}{\mathcal{N}}
\newcommand{\calO}{\mathcal{O}}
\newcommand{\calP}{\mathcal{P}}
\newcommand{\calQ}{\mathcal{Q}}
\newcommand{\calR}{\mathcal{R}}
\newcommand{\calS}{\mathcal{S}}
\newcommand{\calT}{\mathcal{T}}
\newcommand{\calU}{\mathcal{U}}
\newcommand{\calV}{\mathcal{V}}
\newcommand{\calW}{\mathcal{W}}
\newcommand{\calX}{\mathcal{X}}
\newcommand{\calY}{\mathcal{Y}}
\newcommand{\calZ}{\mathcal{Z}}




% \newcommand{\bA}{\mathbf{A}}
% \newcommand{\bB}{\mathbf{B}}
% \newcommand{\bC}{\mathbf{C}}
% \newcommand{\bD}{\mathbf{D}}
% \newcommand{\bE}{\mathbf{E}}
% \newcommand{\bF}{\mathbf{F}}
% \newcommand{\bG}{\mathbf{G}}
% \newcommand{\bH}{\mathbf{H}}
% \newcommand{\bI}{\mathbf{I}}
% \newcommand{\bJ}{\mathbf{J}}
% \newcommand{\bK}{\mathbf{K}}
% \newcommand{\bL}{\mathbf{L}}
% \newcommand{\bM}{\mathbf{M}}
% \newcommand{\bN}{\mathbf{N}}
% \newcommand{\bO}{\mathbf{O}}
% \newcommand{\bP}{\mathbf{P}}
% \newcommand{\bQ}{\mathbf{Q}}
% \newcommand{\bR}{\mathbf{R}}
% \newcommand{\bS}{\mathbf{S}}
% \newcommand{\bT}{\mathbf{T}}
% \newcommand{\bU}{\mathbf{U}}
% \newcommand{\bV}{\mathbf{V}}
% \newcommand{\bW}{\mathbf{W}}
% \newcommand{\bX}{\mathbf{X}}
% \newcommand{\bY}{\mathbf{Y}}
% \newcommand{\bZ}{\mathbf{Z}}
% \newcommand{\ba}{\mathbf{a}}
% \newcommand{\bb}{\mathbf{b}}
% \newcommand{\bc}{\mathbf{c}}
% \newcommand{\bd}{\mathbf{d}}
% \newcommand{\be}{\mathbf{e}}
% \newcommand{\bk}{\mathbf{k}}
% \newcommand{\bmf}{\mathbf{f}}
% \newcommand{\bu}{\mathbf{u}}
% \newcommand{\bp}{\mathbf{p}}
% \newcommand{\bs}{\mathbf{s}}
% \newcommand{\bg}{\mathbf{g}}
% \newcommand{\bh}{\mathbf{h}}
% \newcommand{\br}{\mathbf{r}}
% \newcommand{\bv}{\mathbf{v}}
% \newcommand{\bq}{\mathbf{q}}
% \newcommand{\bx}{\mathbf{x}}
% \newcommand{\by}{\mathbf{y}}
% \newcommand{\bz}{\mathbf{z}}
% \newcommand{\bxi}{{\bm{\xi}}}
\newcommand{\diag}{\mathop{\rm{diag}}}
\newcommand{\Max}{\mathop{\rm Max}}
\newcommand{\Min}{\mathop{\rm Min}}
\newcommand{\argmin}{\mathop{\mathrm{argmin}}}  
\newcommand{\argmax}{\mathop{\mathrm{argmax}}}  
\newcommand{\Var}{\mathop{\mathrm{Var}}}
\newcommand{\Sigmoid}{\mathop{\rm{Sigmoid}}}
\newcommand{\Softmax}{\mathop{\rm{Softmax}}}
\newcommand{\Sparsemax}{\mathop{\rm{Sparsemax}}}
\newcommand{\Sign}{\mathop{\rm{Sign}}}
\newcommand{\lse}{\mathop{\rm{lse}}}



\newcommand{\sumN}{\sum_{i=1}^N}
\newcommand{\sumK}{\sum_{k=1}^K}
\newcommand{\sumq}{\sum_{k=1}^q}
\newcommand{\summ}{\sum_{i=1}^m}
\newcommand{\sumM}{\sum_{\mu=1}^M}
\newcommand{\sumn}{\sum_{i=1}^n}
\newcommand{\sumd}{\sum_{i=1}^d}
\newcommand{\sumT}{\sum_{t=1}^T}

\def\P{\mathbb{P}}
\def\R{\mathbb{R}}
\def\B{\mathbb{B}}
\def\E{\mathbb{E}}
\def\I{\mathcal{I}}
\def\p{\partial }
\let\cite\citep 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\usepackage{amsthm}
%%% make remark better %%%
\makeatletter
\def\th@remark{%
  \thm@headfont{\bfseries}%
  \normalfont % body font
  \thm@preskip\topsep \divide\thm@preskip\tw@
  \thm@postskip\z@ % no extra spacing below
}
\makeatother
% 
% \usepackage[standard,hyperref,amsmath]{ntheorem}
\usepackage[many]{tcolorbox}
\theoremstyle{definition}
\newtheorem{theorem}{Theorem}[section]
\tcolorboxenvironment{theorem}{
  breakable,
  colback=black!10,
  colframe=white,%
  width=\dimexpr\linewidth+10pt\relax,%  
  enlarge left by=-5pt,%                  
  enlarge right by=-5pt,%                 
  boxsep=5pt,%            
  boxrule=0pt,
  left=0pt,right=0pt,top=0pt,bottom=0pt,
  % oversize=2pt,
  sharp corners,
  before skip=\topsep,
  after skip=\topsep
}
\newtheorem{lemma}{Lemma}[section]
\tcolorboxenvironment{lemma}{
  breakable,
  colback=black!10,
  colframe=white,%
  width=\dimexpr\linewidth+10pt\relax,%  
  enlarge left by=-5pt,%                  
  enlarge right by=-5pt,%                 
  boxsep=5pt,%            
  boxrule=0pt,
  left=0pt,right=0pt,top=0pt,bottom=0pt,
  % oversize=2pt,
  sharp corners,
  before skip=\topsep,
  after skip=\topsep
}
\newtheorem{corollary}{Corollary}[theorem]
\tcolorboxenvironment{corollary}{
  breakable,
  colback=black!10,
  colframe=white,%
  width=\dimexpr\linewidth+10pt\relax,%  
  enlarge left by=-5pt,%                  
  enlarge right by=-5pt,%                 
  boxsep=5pt,%            
  boxrule=0pt,
  left=0pt,right=0pt,top=0pt,bottom=0pt,
  % oversize=2pt,
  sharp corners,
  before skip=\topsep,
  after skip=\topsep
}
\newtheorem{proposition}{Proposition}[section]
\theoremstyle{definition}
\newtheorem{definition}{Definition}[section]
\tcolorboxenvironment{definition}{
  breakable,
  colback=black!10,
  colframe=white,%
  width=\dimexpr\linewidth+10pt\relax,%  
  enlarge left by=-5pt,%                  
  enlarge right by=-5pt,%                 
  boxsep=5pt,%            
  boxrule=0pt,
  left=0pt,right=0pt,top=0pt,bottom=0pt,
  % oversize=2pt,
  sharp corners,
  before skip=\topsep,
  after skip=\topsep
}
% \theoremstyle{definition}
\newtheorem{remark}{Remark}[section]
\newtheorem{assumption}{Assumption}[section]
\tcolorboxenvironment{assumption}{
  breakable,
  colback=black!10,
  colframe=white,%
  width=\dimexpr\linewidth+10pt\relax,%  
  enlarge left by=-5pt,%                  
  enlarge right by=-5pt,%                 
  boxsep=5pt,%            
  boxrule=0pt,
  left=0pt,right=0pt,top=0pt,bottom=0pt,
  % oversize=2pt,
  sharp corners,
  before skip=\topsep,
  after skip=\topsep
}
\newtheorem{problem}{Problem}
\tcolorboxenvironment{problem}{
  breakable,
  colback=black!10,
  colframe=white,%
  width=\dimexpr\linewidth+10pt\relax,%  
  enlarge left by=-5pt,%                  
  enlarge right by=-5pt,%                 
  boxsep=5pt,%            
  boxrule=0pt,
  left=0pt,right=0pt,top=0pt,bottom=0pt,
  % oversize=2pt,
  sharp corners,
  before skip=\topsep,
  after skip=\topsep
}
\newtheorem{proc}{Procedure}
\newtheorem{property}{Property}

\crefname{theorem}{Theorem}{Theorems}
\crefname{proposition}{Proposition}{Propositions}
\crefname{lemma}{Lemma}{Lemmas}
\crefname{corollary}{Corollary}{Corollaries}
\crefname{definition}{Definition}{Definitions}
\crefname{assumption}{Assumption}{Assumptions}
\crefname{remark}{Remark}{Remarks}
\crefname{problem}{Problem}{Problems}
\crefname{property}{Property}{property}
\newtheorem{hypothesis}{Hypothesis}
\tcolorboxenvironment{hypothesis}{
  breakable,
  colback=black!10,
  colframe=white,%
  width=\dimexpr\linewidth+10pt\relax,%  
  enlarge left by=-5pt,%                  
  enlarge right by=-5pt,%                 
  boxsep=5pt,%            
  boxrule=0pt,
  left=0pt,right=0pt,top=0pt,bottom=0pt,
  % oversize=2pt,
  sharp corners,
  before skip=\topsep,
  after skip=\topsep
}
\crefname{hypothesis}{Hypothesis}{Hypothesises}

\newtheorem{fact}{Fact}
\tcolorboxenvironment{fact}{
  breakable,
  colback=black!10,
  colframe=white,%
  width=\dimexpr\linewidth+10pt\relax,%  
  enlarge left by=-5pt,%                  
  enlarge right by=-5pt,%                 
  boxsep=5pt,%            
  boxrule=0pt,
  left=0pt,right=0pt,top=0pt,bottom=0pt,
  % oversize=2pt,
  sharp corners,
  before skip=\topsep,
  after skip=\topsep
}
\crefname{fact}{Fact}{Facts}

\newtheorem{example}{Example}
\tcolorboxenvironment{example}{
  breakable,
  colback=black!10,
  colframe=white,%
  width=\dimexpr\linewidth+10pt\relax,%  
  enlarge left by=-5pt,%                  
  enlarge right by=-5pt,%                 
  boxsep=5pt,%            
  boxrule=0pt,
  left=0pt,right=0pt,top=0pt,bottom=0pt,
  % oversize=2pt,
  sharp corners,
  before skip=\topsep,
  after skip=\topsep
}
\crefname{example}{Example}{Examples}

\newtheorem{question}{Question}
\tcolorboxenvironment{question}{
  breakable,
  colback=black!10,
  colframe=white,%
  width=\dimexpr\linewidth+10pt\relax,%  
  enlarge left by=-5pt,%                  
  enlarge right by=-5pt,%                 
  boxsep=5pt,%            
  boxrule=0pt,
  left=0pt,right=0pt,top=0pt,bottom=0pt,
  % oversize=2pt,
  sharp corners,
  before skip=\topsep,
  after skip=\topsep
}
\crefname{question}{Question}{Questions}

\numberwithin{equation}{section}
\numberwithin{theorem}{section}
\numberwithin{proposition}{section}
\numberwithin{definition}{section}
\numberwithin{lemma}{section}
\numberwithin{assumption}{section}
\numberwithin{remark}{section}

%=== footnote without marker ===
% \blfootnote[]{}
\usepackage{lipsum}

\newcommand\blfootnote[1]{%
  \begingroup
  \renewcommand\thefootnote{}\footnote{#1}%
  \addtocounter{footnote}{-1}%
  \endgroup
}
%=== footnote without marker ===
%%% derivation step description
\newcommand*{\annot}[1]{\tag*{\footnotesize{\textcolor{black!50}{\big(#1\big)}}}}

%%% Better Bar Notation%%%
\makeatletter
\let\save@mathaccent\mathaccent
\newcommand*\if@single[3]{%
    \setbox0\hbox{${\mathaccent"0362{#1}}^H$}%
    \setbox2\hbox{${\mathaccent"0362{\kern0pt#1}}^H$}%
    \ifdim\ht0=\ht2 #3\else #2\fi
}
%The bar will be moved to the right by a half of \macc@kerna, which is computed by amsmath:
\newcommand*\rel@kern[1]{\kern#1\dimexpr\macc@kerna}
%If there's a superscript following the bar, then no negative kern may follow the bar;
%an additional {} makes sure that the superscript is high enough in this case:
\newcommand*\widebar[1]{\@ifnextchar^{{\wide@bar{#1}{0}}}{\wide@bar{#1}{1}}}
%Use a separate algorithm for single symbols:
\newcommand*\wide@bar[2]{\if@single{#1}{\wide@bar@{#1}{#2}{1}}{\wide@bar@{#1}{#2}{2}}}
\newcommand*\wide@bar@[3]{%
    \begingroup
    \def\mathaccent##1##2{%
        %Enable nesting of accents:
        \let\mathaccent\save@mathaccent
        %If there's more than a single symbol, use the first character instead (see below):
        \if#32 \let\macc@nucleus\first@char \fi
        %Determine the italic correction:
        \setbox\z@\hbox{$\macc@style{\macc@nucleus}_{}$}%
        \setbox\tw@\hbox{$\macc@style{\macc@nucleus}{}_{}$}%
        \dimen@\wd\tw@
        \advance\dimen@-\wd\z@
        %Now \dimen@ is the italic correction of the symbol.
        \divide\dimen@ 3
        \@tempdima\wd\tw@
        \advance\@tempdima-\scriptspace
        %Now \@tempdima is the width of the symbol.
        \divide\@tempdima 10
        \advance\dimen@-\@tempdima
        %Now \dimen@ = (italic correction / 3) - (Breite / 10)
        \ifdim\dimen@>\z@ \dimen@0pt\fi
        %The bar will be shortened in the case \dimen@<0 !
        \rel@kern{0.6}\kern-\dimen@
        \if#31
        \overline{\rel@kern{-0.6}\kern\dimen@\macc@nucleus\rel@kern{0.4}\kern\dimen@}%
        \advance\dimen@0.4\dimexpr\macc@kerna
        %Place the combined final kern (-\dimen@) if it is >0 or if a superscript follows:
        \let\final@kern#2%
        \ifdim\dimen@<\z@ \let\final@kern1\fi
        \if\final@kern1 \kern-\dimen@\fi
        \else
        \overline{\rel@kern{-0.6}\kern\dimen@#1}%
        \fi
    }%
    \macc@depth\@ne
    \let\math@bgroup\@empty \let\math@egroup\macc@set@skewchar
    \mathsurround\z@ \frozen@everymath{\mathgroup\macc@group\relax}%
    \macc@set@skewchar\relax
    \let\mathaccentV\macc@nested@a
    %The following initialises \macc@kerna and calls \mathaccent:
    \if#31
    \macc@nested@a\relax111{#1}%
    \else
    %If the argument consists of more than one symbol, and if the first token is
    %a letter, use that letter for the computations:
    \def\gobble@till@marker##1\endmarker{}%
    \futurelet\first@char\gobble@till@marker#1\endmarker
    \ifcat\noexpand\first@char A\else
    \def\first@char{}%
    \fi
    \macc@nested@a\relax111{\first@char}%
    \fi
    \endgroup
    }
\makeatother
\let\bar\widebar


%%% sin, cos parentheses %%% 
\makeatletter
\newcommand*{\redefinesymbolwitharg}[1]{%
  \expandafter\let\csname ltx#1\expandafter\endcsname\csname #1\endcsname
  \@namedef{#1}{\@ifnextchar{^}{\@nameuse{#1@}}{\@nameuse{#1@}^{}}}%
  \expandafter\def\csname #1@\endcsname^##1##2{%
     \csname ltx#1\endcsname\ifx!##1!\else^{##1}\fi\mathopen{}\mathclose\bgroup\left(##2\aftergroup\egroup\right)
     }%
}
\makeatother
\redefinesymbolwitharg{sin}
\redefinesymbolwitharg{cos}
%%% sin, cos parentheses %%% 
